'Don't Get Too Technical with Me': A Discourse Structure-Based Framework for Science Journalism

Science journalism refers to the task of reporting technical findings of a scientific paper as a less technical news article to the general public audience. We aim to design an automated system to support this real-world task (i.e., automatic science journalism) by 1) introducing a newly-constructed and real-world dataset (SciTechNews), with tuples of a publicly-available scientific paper, its corresponding news article, and an expert-written short summary snippet; 2) proposing a novel technical framework that integrates a paper's discourse structure with its metadata to guide generation; and, 3) demonstrating with extensive automatic and human experiments that our framework outperforms other baseline methods (e.g. Alpaca and ChatGPT) in elaborating a content plan meaningful for the target audience, simplifying the information selected, and producing a coherent final report in a layman's style.

==> prev-forms.tex <==


% \subsection{Task Formulation}
% Given a text dataset exhibiting an specific writing style, the data is assumed to be generated by the following process
% \begin{itemize}
%     \item a latent style variable $s$ is generated from some distribution  $p(s)$
%     \item a latent content variable $z$ is generated from some distribution $p(z)$
%     \item a latent discrete variable $a \ in \mathcal{A}$, denoting content category, is generated from conditional distribution $p(a|z)$
%     \item a datapoint $x$ is generated from conditional distribution $p(x|s,z,a)$
% \end{itemize}
% Let two datasets, $X^1$ and $X^2$, be observed with the same content distribution but different styles $s_1$ and $s_2$, where $s_1$ and $s_2$ are unknown.
% We say that samples from $X^1$ were drawn from $p(x_1|s_1)$ and samples from $X^2$, from $p(x_2|s_2)$.

% Now, we posit the problem of scientific journalism as follows.
% Let style $s_1$ denote the scientific style used in scientific articles, and $s_2$ the journalistic style used in press release articles.
% Then, let $\mathcal{D}=\langle x_0,x_1,...,x_N \rangle$ be a document in style $s_1$,
% paired with two corresponding summary texts, $\mathcal{Y}^1=\langle y^1_0,...,y^2_{M_1}\rangle$ in style $s_1$
% and $\mathcal{Y}^2=\langle y^2_0,...,y^2_{M_2}\rangle$ in style $s_2$, where these are all sequences of sentences and $M_1$ and $M_2$ are the number of sentences in $\mathcal{Y}^1$ and $\mathcal{Y}^2$, respectively.

% Then, the task of scientific journalism consists on generating a summary in press release style, $\mathcal{Y}^2$,
% given the complete body of a scientific article, $\langle \mathcal{D},\mathcal{M},\mathcal{Y}^1 \rangle$,
% where $\mathcal{M}$ is metadata information of the article, e.g.\ authors and affiliations.
% We now elaborate on the models proposed for this task.


% \subsection{Model}
% \paragraph{Content Planning}
% The first proposed model guides generation of the target summary through a content plan in the form of a sequence of content category values.
% Given $\langle \mathcal{D},\mathcal{Y}^1 \rangle$, the model operates in three steps.
% First, an encoding step infers each sentence $x_i$'s content $z_i \sim p(z_i|x_i,s_1)$ and content category $a_i \in \mathcal{A}$, as follows
% \begin{align}
%     z_i & = E_z(x_i,z_{<i},s_1) \\
%     p(a_i|z_i,s_1) & = softmax(E_a(z_i,s_1))    
% \end{align}
% %\noindent where E() is an

% Second, content in $\mathcal{D}$ is organized in groups, $C_k=\{ z_i ; a_i=k\}$, and
% content plan for $\mathcal{Y}^2$ is generated $B=\langle b_0,...b_{M_2} \rangle, b_j \in \mathcal{A}$,
% \begin{align}
%     q_j & = G_z(c_j,s_2,q_{j-1}) \\
%     p(b_j|b_{<j}) & = softmax(q_j)
% \end{align}
% \nointend where $c_j$ is the attention vector calculated over all groups $C_*$.
% Finally, generation of sentence $y_j=\langle y^0_j,...,y^{|y_j|}_j \rangle, y_j \in \mathcal{Y}^2$ is conditioned on plan $B$ and target style $s_2$, as follows
% \begin{align}
%     h^t_j & = G_y(h^{t-1}_j,b_j,s_2) \\
%     p(y^t_j|y^{<t}_j) & = softmax(h^t_j)
% \end{align}

% \paragraph{Content and Style Planning}
% In addition to plan what content we will include, the second proposed model leverages linguistic templates in order to guide the style realization in each target sentence.
% Each template has the form ....
% Encoding of the input document and grouping of content representation proceeds as before but the guiding plan now also includes a sequence of template labels $P=\langle p_0,...p_{M_2} \rangle, p_j \in \mathcal{P}$,
% \begin{align}
%     q^z_j & = D_z(c_z,q^p_{j-1},q^z_{j-1}) \\
%     q^p_j & = D_p(c_z,q^p_{j-1},q^z_{j-1},s_2) \\
%     p(b_j|b_{<j}) & = softmax(q^z_j) \\
%     p(p_j|p_{<j}) & = softmax(q^p_j)
% \end{align}
% Then, generation of target sentence $y_j=\langle y^0_j,...,y^{|y_j|}_j \rangle, y_j \in \mathcal{Y}^2$ proceeds as follows
% \begin{align}
%     h^t_j & = D_y(h^{t-1}_j,q^z_j,q^p_j,s_2) \\
%     p(y^t_j|y^{<t}_j) & = softmax(h^t_j)
% \end{align}


% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\textwidth]{modules.png}
%     \caption{Modules of content and style planning models.}
%     \label{fig:red-bin}
% \end{figure*}


% \subsection{Training}

% When applying to the same style, the pipeline in Figure X can be simplified into an autoencoder.
% Hence, we define the 

% \begin{align}
%     \mathcal{L}_{rec} &= \mathbb{E}_{Y^1 \sim X^1} [-log p_{G_y}(y^1_j|s_1,E_za(E^1(y^1_j,s_1)))] + \\
%     & \mathbb{E}_{Y^2 \sim X^2} [-log p_{G_y}(y^1_j|s_1,C'(E_a(y^1_j,s_1)))] +
% \end{align}



% \begin{algorithm}
% \caption{Memory simulation by \textsc{GraphKvD}}\label{alg:graphkvd}
% \small
% \begin{algorithmic}[1]
% \Require $\mathcal{D}$, source document as a list of sentences
% \Require $\mathtt{WM}$, size of working memory
% \Require $\mathtt{\Psi}$, maximum tree persistence
% \State $T \gets \emptyset$
% \State $G \gets \emptyset$
% \State $\psi \gets 0$
% \For{$s_k$ in $\mathcal{D}$}
%     \State $P_k \gets getPropositionTree(s_k)$
%     \State $G',attached \gets attachPropositions(P_k,T,G)$
%     \If{$attached$ is True}
%         \State $updateGraph(G',G)$
%         \State $T' \gets getMaximumSpanningTree(G')$
%         \State $T'' \gets memorySelect(\mathtt{WM},T',G)$
%         \State $updateScore(T'')$
%         \State $\psi \gets 0$
%         \State $T \gets T''$
%     \Else
%         \State $\psi \gets \psi + 1$
%     \EndIf
%     \If{ $\psi = \Psi$ }
%         \State $T \gets \emptyset$
%     \EndIf
% \EndFor
% \end{algorithmic}
% \end{algorithm}



% \subsection{Potential tasks}

% \textsc{ACM TechNews} pairs informative texts in two different styles, newswire and scientific, each side with
% with increasing levels of content granularity --main article, summary, and title.
% This scenario opens the possibility to investigate a wide range of interesting tasks related to summarization, style transfer, and text simplification. We now compare our dataset against benchmarks in each of these tasks.


% \paragraph{Summarization.}
% The task of single-document summarization consists on consuming a source text document and generate a shorter text with the gist of the information, maintaining the output summary coherent, relevant, and non-redundant.
% Table~\ref{table:stats} compares \textsc{ACM TechNews} against summarization datasets for newswire and scientific domains. 
% In addition to provide another benchmark for summarization of scientific literature, our dataset enables the task of \textit{press release summarization}.
% This task can be considered a sub-task of newswire summarization where the domain is narrowed down to technological advancements reported in press releases.

% \paragraph{Text Simplification.}
% % not sure whether to call it TS or style transfer
% Text simplification consists on generating a version of a source document which is easier to read and understand.
% Notably, the simplified version can be shorter or longer than its original.
% The \textsc{ACM TechNews} dataset, however, allows for simplification of a scientific article into a press release article.
% In order to avoid extreme compression rates, we investigate the simplification of comparable article parts between both aspects, i.e.\ Sc-title to Nw-title (which could be thought as headline generation), Sc-abstract to Nw-summary, and Sc-body to Press Release body.


==> rebutal.tex <==

We appreciate the constructive comments from the action editor and the reviewers, which helped significantly improve the paper.
Below you can find our response to each of the action editor and reviewer comments. The main changes that we made are as follows:
We have now added these details into the main text.

\section{Reviewer 1}

\paragraph{Human evaluation campaign.}
Participants were selected so that their area of expertise do not overlap significantly with the topic of the articles in the study.
Each participant annotated all 30 articles but were allowed to do so in their own pace and time.
Moreover, we discouraged participants from doing more than 5 articles in a single sitting in order to minimize aggregated cognitive load.
Regarding inter-annotator agreement was found to be XX by means of XX method.
For the factuality criteria, we consider the following name entities: names of people, locations, organization, as well as numbers.
We limit our analysis to intrinsic factuality --cite here--, by which we define a summary as factual if the named entities in it 
can be found in the source document.
A candidate summary is less factual than another if it presents more incorrect named entities.
When two summaries have the same amount of correct or incorrect entities, participants were instructed to annotated them as a tie.

\paragraph{BertScore in technical domains.}
Previous work  has shown that BertScore with in-domain importance weighting is a reliable metric for semantic relevance for highly technical domains such as medical texts \cite{miura2021improving} or informal-language setups such as social media [1].
In this work, we report BertScore values using in-domain importance weighting.

%% improve related section

\paragraph{Ethics Statement.} Thank you for the suggestion. An example scenario has now been added.

%% DONT QUITE WHAT THEY MEAN BY THIS
% It may be helpful to clarify the role of press releases in science journalism (which sometimes are written more for pickup by journalists) compared to news articles written for the broader public, and where ACM TechNews falls on this spectrum.

\paragraph{Prompts for LLMs.} We also tried the following prompts
% add here % 
but they underperformed during preliminary experiments.

\paragraph{Related section and dataset references.} Thank you for the helpful references. We have now added them to the discussion.

\paragraph{Figures.} we will add patterns to Figure 3 and 4 for color-blind friendly readability.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Reviewer 2}

% "a more absolute measure of the accuracy and completeness of the lay summaries"
\paragraph{Evaluation of utility of generated summaries.}

we will run additional study asking for "utility as press release summary"
this would be equivalent to "Overall" category in other human studies.


\paragraph{Test of Statistical Significance.}
-- calculate p vals --
we employed boostrapping with a confidence interval of $95\%$ and $p<XX$ 
Differences in values of readability metrics can indeed be significant up to the second decimal, as reported by previous work [2]
The same can be said about BertScore [3]

\paragraph{Meta outperforming Plan.}
the difference in summary lengths makes evaluation too unreliable, I suppose.
we could run another study this time limiting the number of sentences, number of tokens, or number of bytes
- #sents (memsum)
- #tokens (bigpatent)
- #bytes (reinforce-shashi)

\paragraph{Licence of ACM TechNews data.}
Press release snippets are released under a non-commercial licence.

\paragraph{Number of scientific articles.}
ACM TechNews not only reports on the latest published scientific articles but also about economical, financial, and even political trends.
For this reason, the fraction of snippets linking to a scientific article is small.

\paragraph{Training procedure.}
training was done over the validation set.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Reviewer 3}

\paragraph{Control with user plans.}
add example with different plans

\paragraph{Using GPT3.5 and GPT-4.}
we appreciate the suggestion but we argue that it is not scientifically sound to benchmark `closed' models,
i.e.\ systems for which no details on their training, inference, or even architecture are openly available.
At the time of writing, Alpaca was deemed competitive to closed OpenAI systems and hence we consider it a valid comparison system.

\paragraph{Dataset statistics.}
In total, we gathered 29,069 press release summaries from the main ACM TechNews feed.
However, this feed also contains summaries not related to scientific articles or discoveries but rather economic, financial, and even political trends.
Hence, only 18,933 summaries were related to press release articles of scientific articles.



[1] \cite{hossain2020covidlies}
[2] goldsack
[3] Re-evaluating Evaluation in Text Summarization


